Y-CA-Net: A Convolutional Attention Based Network for Volumetric Medical Image Segmentation

Recent attention-based volumetric segmentation (VS) methods have achieved remarkable performance in the medical domain which focuses on modeling long-range dependencies. However, for voxel-wise prediction tasks, discriminative local features are key components for the performance of the VS models which is missing in attention-based VS methods. Aiming at resolving this issue, we deliberately incorporate the convolutional encoder branch with transformer backbone to extract local and global features in a parallel manner and aggregate them in Cross Feature Mixer Module (CFMM) for better prediction of segmentation mask. Consequently, we observe that the derived model, Y-CT-Net, achieves competitive performance on multiple medical segmentation tasks. For example, on multi-organ segmentation, Y-CT-Net achieves an 82.4% dice score, surpassing well-tuned VS Transformer/CNN-like baselines UNETR/ResNet-3D by 2.9%/1.4%. With the success of Y-CT-Net, we extend this concept with hybrid attention models, that derived Y-CH-Net model, which brings a 3% improvement in terms of HD95 score for same segmentation task. The effectiveness of both models Y-CT-Net and Y-CH-Net verifies our hypothesis and motivates us to initiate the concept of Y-CA-Net, a versatile generic architecture based upon any two encoders and a decoder backbones, to fully exploit the complementary strengths of both convolution and attention mechanisms. Based on experimental results, we argue Y-CA-Net is a key player in achieving superior results for volumetric segmentation.

==> figures/bargraph.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=0.48
\textwidth]{figures/bargraph-updated.png}
\end{center}
\vspace{-2em}
\caption{Comparison of performance of UNETR with ResNet-3D on Synapse dataset. ResNet-3D is consistently performing better than UNETR in all organs.}
\vspace{-1.0em}
\label{fig:bargraph}
\end{figure}

==> figures/combine-comparison.tex <==

\begin{figure*}[!ht]

\begin{minipage}{\textwidth}
\begin{minipage}{0.48\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/bargraph.png}
\vspace{-2em}
\caption{\footnotesize Quantitative comparison of performance of ViT with ResNet-3D on Synapse dataset in UNETR settings. ResNet-3D is consistently performing better than ViT in all organs.}\label{fig:bargraph}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\centering
\begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
    \includegraphics[ height=2.4cm, width=1.3\linewidth]{new-figures/label-updated.png}
  \end{minipage}
  ~~~~~~
  \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
   \includegraphics[height=2.4cm, width=1.3\linewidth]{new-figures/resnetgt-updated.png}
  \end{minipage}
  ~~~~~~
\begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up
  \includegraphics[height=2.4cm, width=1.3\linewidth]{new-figures/unetrgt-updated.png}
  \end{minipage}\\
~~~~~~~\footnotesize Label ~~~~~~~~~~~~~~~~~~~~~~~ \footnotesize ConvNet ~~~~~~~~~~~~~~~~~~~~~~~~~  \footnotesize ViT
\caption{
\footnotesize Qualitative Comparison of ViT Encoder and ResNet-3D Encoder in UNETR settings with ground truth label. The difference is clearly shown in the segmentation mask which is highlighted by small square boxes. }\label{fig:visualizations}
  \end{minipage}
    \end{minipage}
\vspace{-1em}
\end{figure*}

==> figures/comparsion.tex <==
\begin{figure}
\begin{minipage}{0.46\textwidth}
\centering
\begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
    \includegraphics[height=2.2cm, width=1.2\linewidth]{figures/GroundTruth.png}
     \footnotesize GT
  \end{minipage}
  ~~~~
  \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
   \includegraphics[height=2.2cm, width=1.2\linewidth]{figures/Resnet-pred.png}
   \footnotesize ResNet-3D
  \end{minipage}
  ~~~~
\begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up
  \includegraphics[height=2.2cm, width=1.2\linewidth]{figures/unetr-pred.png}
  \footnotesize ViT
  \end{minipage}
\caption{ \footnotesize{Qualitative Comparison of ViT Encoder and ResNet-3D Encoder in UNETR settings with ground truth. The clear difference is shown highlighted by the arrow key.}}\label{fig:visualizations}
  \end{minipage}

\end{figure}

==> figures/concept-diagram.tex <==
%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=0.45\textwidth]{figures/Concept-Diagra.png}
%\end{center}
%\vspace{-3em}
%\caption{\footnotesize Overview of our proposed hybrid method HCT-Net. Our proposed framework consists of two encoder networks: CNN and transformer extract local and global features independently from 3D volume which are mixed in Cross Feature Mixture Module and output is passed to a ConvNet-based decoder for dense prediction.}
%\vspace{-2.0em}
%\label{fig:concept-diagram}
%\end{figure}



==> spleen-results/spleen-results.tex <==
\begin{figure*}[!ht]
\begin{minipage}{0.5\textwidth}
\centering
%\vspace{0.2em}
\begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
    \includegraphics[height=2.4cm, width=\linewidth]{spleen-results/gt.png}
    \textbf{LABEL}
  \end{minipage}
  \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
   \includegraphics[height=2.4cm, width=\linewidth]{spleen-results/lgmixer-gt.png}
   \textbf{LGMiXer}
  \end{minipage}
\begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up
  \includegraphics[height=2.4cm, width=\linewidth]{spleen-results/swinunetr-gt.png}
  \textbf{Swin-UNETR}
  \end{minipage}
  \begin{minipage}{0.24\textwidth}
      \centering
       % lelf lower right up trim= 7.5mm 0mm 0mm 10mm
    \includegraphics[height=2.4cm, width=\linewidth]{spleen-results/unetr-gt.png}
    \textbf{UNETR}
  \end{minipage}
\caption{ \footnotesize{Qualitative results on different MSD segmentation tasks. }}\label{fig:visualization-msd}
  \end{minipage}
\end{figure*}\vspace{-1em}

==> tables/ablation-study-2.tex <==
\iffalse
\begin{table}[!ht]
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
\rowcolor{gray!50}
\textbf{Feature Pairs}  & \textbf{Spatial Dimension} &\textbf{Accuracy} \\
\midrule
($\mathcal{F}_{L_{2}}$, $\mathcal{F}_{G_{3}}$) & (24 $\times$ 24 $\times$ 24), (24 $\times$ 24 $\times$ 24) & \textbf{0.824}\\
($\mathcal{F}_{L_{3}}$, $\mathcal{F}_{G_{3}}$) & (12 $\times$ 12 $\times$ 12), (24 $\times$ 24 $\times$ 24) & 0.807\\
($\mathcal{F}_{L_{4}}$, $\mathcal{F}_{G_{3}}$) &  ($\phantom{0}$6 $\times$ $\phantom{0}$6 $\times$ $\phantom{0}$6), (24 $\times$ 24 $\times$ 24)& 0.798\\
($\mathcal{F}_{L_{5}}$, $\mathcal{F}_{G_{3}}$) &  ($\phantom{0}$3 $\times$ $\phantom{0}$3 $\times$ $\phantom{0}$3), (24 $\times$ 24 $\times$ 24) & 0.791\\
\bottomrule

\end{tabular}}
\caption{Ablation study of using different feature pairs used in cross feature mixture module from local and global encoder network to analyze its impact on the performance of the proposed method.}\label{table:position_ablation}
\end{table}\vspace{-0.5em}
\fi

==> tables/ablation-study-3.tex <==
\iffalse
\begin{table}[!ht]
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
\rowcolor{gray!50}
\textbf{Feature Pairs}  & \textbf{Spatial Dimension} &\textbf{Accuracy} \\
\midrule
($\mathcal{F}_{L_{2}}$, $\mathcal{F}_{G_{3}}$) & (24$^3$, 24$^3$) & 0.824\\
($\mathcal{F}_{L_{3}}$, $\mathcal{F}_{G_{4}}$) & (12$^3$, 12$^3$) & 0.823 \\
($\mathcal{F}_{L_{2}}$, $\mathcal{F}_{G_{3}}$)
($\mathcal{F}_{L_{3}}$, $\mathcal{F}_{G_{4}}$)&  (24$^3$, 24$^3$)(12$^3$, 12$^3$) & \textbf{0.839}\\

\bottomrule

\end{tabular}}
\caption{Ablation study of using multiple Cross Feature Mixture Module (CFMM) }\label{table:position_CFMM}
\end{table}
\fi

==> tables/ablation-study-5.tex <==
\iffalse
\begin{table}[!ht]
\centering
\resizebox{0.25\linewidth}{!}{
\begin{tabular}{lc}
\toprule
\rowcolor{gray!50}
\textbf{Blocks}  & \textbf{Accuracy} \\
\midrule
{[}2, 2{]} & 0.782 \\
{[}2, 4{]}  & 0.801 \\
{[}4, 4{]} & 0.839 \\
{[}4, 8{]} & 0.841 \\
{[}8, 8{]} & 0.831 \\
{[}4, 16{]} & \textbf{0.862} \\
{[}4, 24{]} & 0.854\\
\bottomrule

\end{tabular}}
\caption{Ablation study of increasing number of blocks of local encoder network for early stages.}
\label{table:blocks_ablation}
\end{table}\vspace{-0.5em}
\fi
